A Skellam Regression Model for Quantifying Positional Value in Soccer

Soccer is undeniably the most popular sport world-wide and everyone from general managers and coaching staff to fans and media are interested in evaluating players' performance. Metrics applied successfully in other sports, such as the (adjusted) +/- that allows for division of credit among a basketball team's players, exhibit several challenges when applied to soccer due to severe co-linearities. Recently, a number of player evaluation metrics have been developed utilizing optical tracking data, but they are based on proprietary data. In this work, our objective is to develop an open framework that can estimate the expected contribution of a soccer player to his team's winning chances using publicly available data. In particular, using data from (i) approximately 20,000 games from 11 European leagues over 8 seasons, and, (ii) player ratings from the FIFA video game, we estimate through a Skellam regression model the importance of every line (attackers, midfielders, defenders and goalkeeping) in winning a soccer game. We consequently translate the model to expected league points added above a replacement player (eLPAR). This model can further be used as a guide for allocating a team's salary budget to players based on their expected contributions on the pitch. We showcase similar applications using annual salary data from the English Premier League and identify evidence that in our dataset the market appears to under-value defensive line players relative to goalkeepers.

==> old.tex <==

Despite the sport's popularity in the United States, public statistical analysis of American football (``football") has lagged behind that of other major sports.  While new statistical research involving player and team evaluation is regularly published in baseball \citep{Albert06, Jensen09, Piette12, Baumer15}, basketball \citep{Kubatko07, Deshpande16}, and hockey \citep{Macdonald11, Gramacy12, Thomas13}, there is limited new research that addresses on-field or player personnel decisions for National Football League (NFL) teams.  Recent work in football addresses topics such as fantasy football \citep{Becker16}, predicting game outcomes \citep{Balreira14}, NFL TV ratings \citep{Grimshaw14}, the effect of ``fan passion'' and league sponsorship on brand recognition \citep{Wakefield12}, and realignment in college football \citep{Jensen14}.  Additionally, with the notable exception of \citet{Lock14}, recent research relating to on-field or player personnel decisions in football is narrowly focused.  For example, \citet{Mulholland14} analyze the success of tight ends in the NFL draft, \citet{Clark13} and \citet{Pasteur14} both provide improved metrics for kicker evaluation, \citet{Martin17} examine the NFL's change in overtime rules, and \citet{Snyder15} focus on discretionary penalties from referees.  Moreover, statistical analysis of football that does tackle on-field or player personnel decisions frequently relies on proprietary and costly data sources, where data quality often depends on potentially biased and publicly unverified human judgment.  This leads to a lack of reproducibility that is well-documented in sports research \citep{Baumer15}. 

In this paper, we posit that (1) objective on-field and player personnel decisions rely on two fundamental categories of statistical analysis in football:  play evaluation and player evaluation, and (2) in order to maintain a standard of objectivity and reproducibility for these two fundamental areas of analysis, researchers must agree on a dataset standard.

\subsection{Previous Work: Evaluating Plays}
\label{sec:prev-work-plays}

Traditionally, yards gained/lost have been used to evaluate the success of a play. However, this point of view strips away the importance of context in football \citep{Carter71, Carroll88}.  For instance, three yards gained on 3rd and 2 are more valuable than three yards gained on 3rd and 7.  This point, that not all yards are created equal, has been the foundation for the development of two approaches for evaluating plays:  expected points and win probability.  The expected points framework uses historical data to find the number of points eventually scored by teams in similar situations, while the win probability framework uses historical data to find how often teams in similar situations win the game.  One can obtain the difference between pre-snap and post-snap values of a play to estimate the value of the play itself  -- expected points added (\(EPA\)) or win probability added (\(WPA\)).  

These approaches have been recently popularized by Brian Burke's work at \url{www.advancedfootballanalytics.com} and ESPN \citep{Burke_EP, ESPN_total_QBR}. \citet*{Burke_EP} and ESPN provide an intuitive explanation for what expected points means, however they do not go into the details of the calculations. ``Nearest neighbors" algorithms have been used to identify similar situations based on down, yards to go, and the yard line to then average over the next points scored \citep{Carter71, Dasarathy}. \citet*{Goldner17} describes a Markov model and uses the absorption probabilities for different scoring events (touchdown, field goal, and safety) to arrive at the expected points for a play. \citet*{Causey15} takes an exact-neighbors approach, finding all plays with a set of identical characteristics, taking the average outcome, and conducting post-hoc smoothing to calculate expected points.

Compared to expected points models, there is considerably more literature on different methodologies for estimating the win probability of a play in football.  \citet*{Goldner17} uses a Markov model, similar to the approach taken by \citet*{Tango07} in baseball, by including the score differential, time remaining, and timeouts to extend the expected points model.  Burke's approach is primarily empirical estimation by binning plays with adjustments and smoothing.  In some published win probability analyses, random forests have been shown to generate well-calibrated win probability estimates \citep{Causey13, Lock14}.  The approach taken by \citet*{Lock14} also considers the respective strengths of the offensive (possession) and defensive (non-possession) teams.

There are many areas of research that build off of these approaches for valuing plays.  For example, analyses of fourth down attempts and play-calling are very popular \citep{Romer06, Alamar10, Goldner12, Quealy}.  This paper focuses on using play evaluation to subsequently evaluate players, and we discuss prior attempts at player evaluation below.

\subsection{Previous Work:  Evaluating Players}
\label{sec:prev-work-players}

Most analysis for comparing players at offensive skill positions such as quarterback (QB), running back (RB), wide receiver (WR), and tight end (TE) relies on the usage of basic box score statistics such as yards gained, number of attempts, etc. Linear combinations of these box score statistics, such as passer rating \citep{Smith73}, are often used to compare players at the same position while taking into account more than just a single box score measure.  Similarly, Pro Football Reference's adjusted net yards per attempt (``ANY/A") expands upon passer rating in that it accounts for sacks and uses a different linear weighting scheme \citep{PFR}. However these measures are not based on \(EPA\) or \(WPA\), so they are not interpretable in terms of points or wins. 

There have been multiple irreproducible attempts at player evaluation with frameworks considering \(EPA\)-like values. \citet*{Schatz03} provides a metric called ``defense-adjusted value over average" which evaluates plays in manner similar to expected points while also accounting for the strength of the opposing defense. However, specifics on the modeling techniques are not disclosed. ESPN's total quarterback rating (``QBR") accounts for the situational contexts a QB faces throughout a game \citep{ESPN_total_QBR, Oliver11}.  ESPN uses the following approach when computing QBR.  First, they determine the degree of success or failure for each play.  Second, they divide credit for each play amongst all players involved.  Third, additional adjustments are made for plays of very little consequence to the game outcome. This approach has several important advantages.  In the first step, the EPA is used to assign an objective value to each play.  Another advantage is that some attempt is made to divide credit for a play's success or failure amongst the players involved.  We loosely follow these steps in our proposed approach for NFL player evaluation. However ESPN's QBR is not directly reproducible since it relies on human judgment and is limited only to QBs.

For positions other than QB, RB, WR, and TE, data are limited, since the NFL does not publicly provide information about which players are on the field for a particular play, the offensive and defensive formations (other than the ``shotgun" formation on offense), or the pre- and post-snap locations of players on the field. With these positions, it is difficult to obtain adequate within-positional comparisons of player value, let alone across-position comparisons. Pro Football Focus assigns grades to every player in each play, but this approach is solely based on human judgment and proprietary to PFF \citep{Eager17}. The only public approach for evaluating players at all positions according to common scale is Pro Football Reference's ``approximate value" (AV) statistic \citep{Drinen}.  Using a combination of objective and subjective analysis, AV attempts to assign a single numerical value to a player's performance in any season since 1950, regardless of the player's position.  AV has some subjective components, such as whether or not a lineman was named to the NFL's ``all-pro" team, and is not interpretable in terms of game outcomes. There are no publicly known attempts for developing a \textit{Wins Above Replacement} (\textit{WAR}) measure for every individual NFL player, as made popular in baseball \citep{Schoenfield12} and other sports \citep{Thomas15}.

\subsection{Our Framework for Evaluating NFL Plays and Players}

In order to properly evaluate players, we need to allocate a portion of a play's value to each player involved \citep{ESPN_total_QBR}. \citet*{Baumer17} details the history of division of credit modeling as a primary driver of research in sports analytics, with origins in evaluating run contributions in baseball.  However, in comparison to baseball, every football play is more complex and interdependent, with the 22 players on the field contributing in many ways and to varying degrees.  A running play depends not only on the running back but the blocking by the linemen, the quarterback's handoff, the defensive matchup, the play call, etc.  A natural approach is to use a regression-based method, with indicators for each player on the field for a play, providing an estimate of their marginal effect.  This type of modeling has become common in basketball and hockey, because it accounts for factors such as quality of teammates and competition \citep{Rosenbaum04, Kubatko07, Macdonald11, Gramacy12, Thomas13}.

We present four contributions to the study of football statistics in order to address the issues pertaining to play evaluation and player evaluation outlined above:

\begin{enumerate}
  \item The \texttt{R} package \texttt{nflscrapR} to provide easy access to publicly available NFL play-by-play data (Section \ref{sec:data}).
  \item A novel approach for estimating expected points using a multinomial logistic regression model, which more appropriately models the ``next score" response variable (Section \ref{sec:ep}).
  \item A generalized additive model for estimating the win probability using the expected points as input (Section \ref{sec:wp}).
  \item Our \textit{nflWAR} framework, using multilevel models to isolate offensive skill player contribution and estimate their \textit{WAR} (Section \ref{sec:nflwar}).  
\end{enumerate}

We use a resampling procedure similar to \citet{Baumer15} to estimate uncertainty in each player's seasonal \textit{WAR}.  Due to the limitations of publicly available data, the primary focus of this paper is on offensive skill position players: QB, RB, WR, and TE.  However, we present a novel metric that serves as a proxy for measuring a team's offensive line performance on rushing plays.  Furthermore, the reproducible framework we introduce in this paper can also be easily extended to estimate \textit{WAR} for all positions given the appropriate data.  Researchers with data detailing which players are on the field for every play can use the framework provided in Section \ref{sec:road_to_war} to estimate \textit{WAR} for players at all positions.

Our \textit{WAR} framework has several key advantages.  First, it is fully reproducible:  it is built using only public data, with all code provided and all data accessible to the public. Second, our expected points and win probability models are well-calibrated. Third, player evaluation with \textit{WAR} is easily interpretable in terms of game outcomes, unlike prior approaches to player evaluation in the NFL discussed above.  The replacement level baseline informs us how many wins a player adds over a readily available player.  This is more desirable than comparing to average from the viewpoint of an NFL front office, as league average performance is still valuable in context \citep{Baumer15}.  Fourth, the multilevel model framework accounts for quality of teammates and competition.  Fifth, although this paper presents \textit{WAR} using our expected points and win probability models for play evaluation, researchers can freely substitute their own approaches for play evaluation without any changes to the framework for estimating player \textit{WAR}. Finally, we recognize the limitations of point estimates for player evaluation and provide estimates of the uncertainty in a player's \textit{WAR}.

\subsection{Play-by-Play Data with \texttt{nflscrapR}}
\label{sec:data}

Facing the challenge of limited publicly available NFL data and the need for a dataset standard, we develop an \texttt{R} package \citep{R17} called \texttt{nflscrapR} \citep{Horowitz17}. This package was inspired largely by other \texttt{R} packages facilitating the access of sports data such as \texttt{nhlscrapR} \citep{Thomas17}, \texttt{pitchRx} \citep{Sievert15}, \texttt{Lahman} \citep{Lahman}, \texttt{openWAR} \citep{Baumer15}, and \texttt{ballR} \citep{Elmore17}.  The results in this paper are generated entirely from play-by-play data accessed with the \texttt{nflscrapR} package. A detailed description of its functionality is provided in our supplementary materials.

\section{Evaluating Plays with Expected Points and Win Probability}
\label{sec:ep_wp_model}

As described in Section \ref{sec:prev-work-plays}, expected points and
win probability are two common approaches for evaluating plays. These
approaches have several key advantages: They can be calculated using
only the NFL's publicly available data, they provide
estimates of a play's value in terms of real game outcomes (i.e. points
and wins), and, as a result, they are easy to understand for both
experts and non-experts.

Below, we introduce our own novel approaches for estimating expected
points ($EP$) and win probability ($WP$) using publicly available
data via \texttt{nflscrapR}.

\subsection{Expected Points}
\label{sec:ep}

While most authors take the average ``next score'' outcome of similar
plays in order to arrive at an estimate of $EP$, we recognize that
certain scoring events become more or less likely in different
situations. As such, we propose modeling the probability for each of
the scoring events directly, as this more appropriately accounts for the
differing relationships between the different categories of the ``next score'' response and the covariates. Once we
have the probabilities of each scoring event, we can trivially estimate
expected points.

\subsubsection{Multinomial Logistic Regression}

To estimate the probabilities of each possible scoring event conditional
on the current game situation, we use multinomial logistic regression.
For each play, we find the next scoring event within the same half (with
respect to the possession team) as one of the seven possible events:
touchdown (7 points), field goal (3 points), safety (2 points), no score
(0 points), opponent safety (-2 points), opponent field goal (-3
points), and opponent touchdown (-7 points). Here, we ignore point after
touchdown (PAT) attempts, and we treat PATs separately in Section
\ref{sec:pat_fg}.

\autoref{next-score-bar} displays the distribution of the different type
of scoring events using data from NFL regular season games between 2009
and 2016, with each event located on the y-axis based on their
associated point value $y$. This data consists of 304,896 non-PAT
plays, excluding QB kneels (which are solely used to run out the clock
and are thus assigned an $EP$ value of zero). The gaps along the
y-axis between the different scoring events reinforce our decision to
treat this as a classification problem rather than modeling the point
values with linear regression. While we use seven points for a touchdown
for simplicity here, our multinomial logistic regression model generates
the probabilities for the events regardless of the point value. This is
beneficial, since it allows us to flexibly handle PATs and two-point
attempts separately. We can easily adjust the point values
associated with touchdowns to reflect changes in the league's scoring
environment.

\begin{figure}[!h]
%% Use the graphics package to insert figures
\centering
\framebox{%
  \begin{minipage}{10pc}
      \vspace{1cm}\par
      next\_score\_barchart.jpeg\par
      \vspace{1cm}
  \end{minipage}}
\caption{Distribution of next scoring events for all plays from 2009-16, with respect to the possession team.}
\label{next-score-bar}
\end{figure}


We denote the covariates describing the game situation for each play as
$\mathbf{X}$, which are presented in our supplementary materials, and the response variable 
\begin{align}
\label{ep-response}
Y \in & \{\textrm{Touchdown}\ (\textbf{7}),\ \textrm{Field Goal}\ (\textbf{3}),\ \textrm{Safety}\ (\textbf{2}),\ \textrm{No Score}\ (\textbf{0}), \nonumber \\ 
&-\textrm{Touchdown}\ (\textbf{-7}),\ -\textrm{Field Goal}\ (\textbf{-3}),\ -\textrm{Safety}\ (\textbf{-2})\}.
\end{align}

The model is specified with six logit transformations relative to the ``No Score''
event with the form
\begin{align}
  \text{log}(\frac{P(Y=Touchdown|\mathbf{X})}{P(Y=No\ Score|\mathbf{X})}) & = \mathbf{X}\cdot \boldsymbol{\beta}_{Touchdown}, \nonumber \\
  \text{log}(\frac{P(Y=Field\ Goal|\mathbf{X})}{P(Y=No\ Score|\mathbf{X})}) & = \mathbf{X}\cdot \boldsymbol{\beta}_{Field\ Goal}, \nonumber \\
  \vdots  \\
  \text{log}(\frac{P(Y=-Touchdown|\mathbf{X})}{P(Y=No\ Score|\mathbf{X})}) & = \mathbf{X}\cdot \boldsymbol{\beta}_{-Touchdown}, \nonumber
\end{align}

\noindent where $\boldsymbol{\beta}_y$ is the corresponding coefficient vector for the type of next scoring event. Using the generated probabilities for each of the possible scoring
events, $P(Y = y|\mathbf{X})$, we simply calculate the expected
points ($EP$) for a play by multiplying each event's predicted
probability with its associated point value \(y\): 

\begin{equation}
\label{ep-formula}
EP = E[Y | \mathbf{X}] = \sum_y y \cdot P(Y=y | \mathbf{X}).
\end{equation}

\hypertarget{model-selection-with-calibration}{%
\subsubsection{Model Selection with
Calibration}
\label{model-selection-with-calibration}}

Since our expected points model uses the probabilities for each scoring
event from multinomial logistic regression, the variables and
interactions selected for the model are determined via calibration
testing, similar to the criteria for evaluating the win probability
model in \citet{Lock14}. The estimated probability for each of the seven
scoring events is binned in five percent increments (20 total possible
bins), with the observed proportion of the event found in each bin. If
the actual proportion of the event is similar to the bin's estimated
probability then the model is well-calibrated. Because we are generating
probabilities for seven events, we want a model that is well-calibrated
across all seven events. To objectively compare different models, we
first calculate for scoring event \(y\) in bin \(b \in \{1,\hdots, B\}\)
its associated error
\begin{equation}
e_{y,b} = |\hat{P_b}(Y=y) - P_b(Y=y)|,
\end{equation}

\noindent where \(\hat{P_b}(Y=y)\) and \(P_b(Y=y)\) are the predicted
and observed probabilities, respectively, in bin \(b\). Then, the
overall calibration error \(e_y\) for scoring event \(y\) is found by
averaging \(e_{y,b}\) over all bins, weighted by the number of plays in
each bin, \(n_{y,b}\); that is
\begin{equation}
e_y = \frac{1}{n_y}\sum_b n_{y,b} e_{y,b},
\end{equation}

\noindent where \(n_y = \sum_b n_{y,b}\). This leads to the model's
calibration error \(e\) as the average of the seven \(e_y\) values,
weighted by the number of plays with scoring event \(y\), \(n_{y}\):
\begin{equation}
e = \frac{1}{n}\sum_y n_y e_y,
\end{equation}

\noindent where \(n = \sum_y n_y\), the number of total plays. This
provides us with a single statistic with which to evaluate models, in
addition to the calibration charts.

We calculate the model calibration error using leave-one-season-out
cross-validation (LOSO CV) to reflect how the \texttt{nflscrapR} package
will generate the probabilities for plays in a season it has not yet
observed. The selected variables and interactions for the model yielding the best LOSO CV calibration results are available in our supplementary materials. \autoref{ep_cal} displays the selected
model's LOSO CV calibration results for each of the seven scoring
events, resulting in \(e \approx 0.013\). The dashed lines along the
diagonal represent a perfect fit, i.e.~the closer to the diagonal points
are the more calibrated the model. Although time remaining is typically
reserved for win probability models \citep{Goldner17}, including the
seconds remaining in the half, as well as the indicator for under two
minutes, improved the model's calibration, particularly with regards to
the ``No Score'' event. We also explored the use of an ordinal logistic regression model which assumes equivalent effects as the scoring value increases, but found the LOSO CV calibration results to be noticeably worse with \(e \approx 0.022\).

Our supplementary materials provides further details on our novel weighting scheme to handle potential issues regarding score differential \citep{BurkeEP} and the difference in drives from the next score without excluding any observations. These materials also cover our use of a separate model for field goals and PAT attempts. 

\begin{figure}[!h]
\centering
\framebox{%
  \begin{minipage}{10pc}
      \vspace{1cm}\par
      ep\_calibration\_plots.jpeg\par
      \vspace{1cm}
  \end{minipage}}
%% A small box in place of a figure
\caption{Expected points model LOSO CV calibration results by scoring event.}
\label{ep_cal}
\end{figure}

\subsubsection{Expected Points by Down and Yard Line}

For reference, \autoref{ep_comp} displays the relationship between the
field position and the $EP$ for our multinomial logistic regression
model available via \texttt{nflscrapR} compared to the previous
relationships found by \citet{Carter71} and \citet{Carroll88}. We
separate the \texttt{nflscrapR} model by down to show its importance,
and in particular the noticeable drop for fourth down plays and how they
exhibit a different relationship near the opponent's end zone as
compared to other downs. To provide context for what is driving the
difference, \autoref{ep_probs_chart} displays the relationship between
each of the next score probabilities and field position by down. Clearly
on fourth down, the probability of a field goal attempt overwhelms the
other possible events once within 50 yards of the opponent's end zone.

\begin{figure}[!h]
\centering
\framebox{%
  \begin{minipage}{11pc}
      \vspace{1cm}\par
      ep\_distance\_down\_plot.jpeg\par
      \vspace{1cm}
  \end{minipage}}
\caption{Comparison of historical models and \texttt{nflscrapR} expected points value, based on distance from opponent's end zone by down.}
\label{ep_comp}
\end{figure}

\begin{figure}[!h]
\centering
\framebox{%
  \begin{minipage}{11pc}
      \vspace{1cm}\par
      ep\_event\_distance\_plot.jpeg\par
      \vspace{1cm}
  \end{minipage}}
%% A small box in place of a figure
\caption{Relationship between next score event probabilities and field position by down.}
\label{ep_probs_chart}
\end{figure}

\subsection{Win Probability}
\label{sec:wp}

Because our primary focus in this paper is in player evaluation, we
model win probability without taking into account the teams playing (i.e.~we do not
include indicators for team strength in the win probability model). As a
result, every game starts with each team having a 50\% chance of
winning. Including indicators for a team's overall, offensive, and/or
defensive strengths would artificially inflate (deflate) the
contributions made by players on bad (good) teams in the models
described in Section \ref{sec:nflwar}, since their team's win
probability would start lower (higher).

Our approach for estimating \(WP\) also differs from the others
mentioned in Section \ref{sec:prev-work-plays} in that we incorporate the
estimated \(EP\) directly into the model by calculating the expected
score differential for a play. Our expected points model already
produces estimates for the value of the field position, yards to go, etc.
without considering which half of the game or score. When including the
variables presented in Table \ref{table-wp-vars}, we arrive at a
well-calibrated \(WP\) model.

\begin{table}
\centering
\caption{Description of selected variables for the win probability model.  Note:  $S$ is the score differential at the current play.}
\label{table-wp-vars}
\begin{tabular}{ p{3cm} p{9cm}}
\hline \\ [-1.5ex]
Variable & Variable description \\ [1ex]
\hline \\ [-1.5ex]
$E[S]$ & Expected score differential = $EP + S$ \\ [1ex]
$s_{g}$ & Number of seconds remaining in game \\ [1ex]
$E[\frac{S}{s_{g} +1}]$ & Expected score time ratio\\ [1ex]
$h$ & Current half of the game (1st, 2nd, or overtime)  \\ [1ex]
$s_h$ & Number of seconds remaining in half \\ [1ex]
$u$ & Indicator for whether or not time remaining in half is under two minutes \\ [1ex]
$t_{off}$ & Time outs remaining for offensive (possession) team \\ [1ex]
$t_{def}$ & Time outs remaining for defensive team \\ [1ex]
\hline
\end{tabular}
\end{table}

\subsubsection{Generalized Additive Model}
\label{gam}

We use a generalized additive model (GAM) to estimate the possession
team's probability of winning the game conditional on the current game
situation. GAMs have several key benefits that make them ideal for
modeling win probability. They allow the relationship between the
explanatory and response variables to vary according to smooth,
non-linear functions. They also allow for linear relationships and can
estimate (both ordered and unordered) factor levels. We find that this
flexible, semi-parametric approach allows us to capture nonlinear
relationships while maintaining the many advantages of using linear
models. Using a logit link function, our \(WP\) model takes the form
\begin{equation}
\text{log}(\frac{P(\mbox{Win})}{P(\mbox{Loss})}) = s(E[S]) + s(s_h)\cdot h + s(E[\frac{S}{s_{g} +1}]) + h \cdot u \cdot t_{off} + h\cdot u \cdot t_{def},
\end{equation}

\noindent where \(s\) is a smooth function while \(h\), \(u\),
\(t_{off}\), and \(t_{def}\) are linear parametric terms defined in \autoref{table-wp-vars}. By taking the
inverse of the logit we arrive at a play's \(WP\).

\hypertarget{win-probability-calibration}{%
\subsubsection{Win Probability
Calibration}\label{win-probability-calibration}}

Similar to the evaluation of the \(EP\) model, we again use LOSO CV to
select the above model yielding the best calibration results.
\autoref{wp_cal} shows the calibration plots by quarter, mimicking the
approach of \citet{Lopez17} and \citet{Yam18}, who evaluate both our
\(WP\) model and that of \citet{Lock14}. The observed proportion of wins
closely matches the expected proportion of wins within each bin for each
quarter, indicating that the model is well-calibrated across all
quarters of play and across the spectrum of possible win probabilities.
These findings match those of \citet{Yam18}, who find ``no obvious
systematic patterns that would signal a flaw in either model.'' An example of a single game's win probability chart is available in our supplementary materials.

\begin{figure}[!h]
\centering
\framebox{%
  \begin{minipage}{10pc}
      \vspace{1cm}\par
      wp\_calibration\_plots.jpeg\par
      \vspace{1cm}
  \end{minipage}}
%% A small box in place of a figure
\caption{Win probability model LOSO CV calibration results by quarter.}
\label{wp_cal}
\end{figure}

\subsection{Expected Points Added and Win Probability Added}
\label{epa-wpa}

In order to arrive at a comprehensive measure of player performance, each
play in a football game must be assigned an appropriate value
\(\delta_{f,i}\) that can be represented as the change from state \(i\)
to state \(f\). We define
\begin{equation}
\label{play-value}
\delta_{f,i} = \boldsymbol{V}_{f} - \boldsymbol{V}_i,
\end{equation}

\noindent where \(\boldsymbol{V}_{f}\) and \(\boldsymbol{V}_{i}\) are
the associated values for the ending and starting states respectively.
We represent these values by either play \(i\)'s expected points
(\(EP_i\)) or win probability (\(WP_i\)).

Plugging our \(EP\) and \(WP\) estimates for the start of play \(i\) and
the start of the following play \(f\) into \autoref{play-value}'s values
for \(\boldsymbol{V}_i\) and \(\boldsymbol{V}_f\) respectively provides
us with the two types of play valuations \(\delta_{f,i}\): (1) the
change in point value as expected points added (\(EPA\)), and (2) the
change in win probability as win probability added (\(WPA\)). For
scoring plays, we use the associated scoring event's value \(y\) as
\(\boldsymbol{V}_f\) in place of the following play's \(EP\) to reflect
that the play's value is just connected to the difference between the
scoring event and the initial state of the play. As an example, during Super Bowl LII the Philadelphia Eagles' Nick Foles received a touchdown when facing fourth down on their opponent's one yard line with thirty-eight seconds remaining in the half. At the start of the play the Eagles' expected points was \(\boldsymbol{V}_{i}\ \approx 2.78\), thus resulting in $EPA \approx 7 - 2.78 = 4.22$. In an analogous calculation, this famous play known as the ``Philly special" resulted in $WPA \approx 0.1266$ as the Eagles' increased their lead before the end of the half.

For passing plays, we can additionally take advantage of \emph{air
yards} (perpendicular distance in yards from the line of scrimmage to
the yard line at which the receiver was targeted or caught the ball) and
\emph{yards after catch} (perpendicular distance in yards from the yard
line at which the receiver caught the ball to the yard line at which the
play ended), for every passing play available with \texttt{nflscrapR}.
Using these two pieces, we can determine the hypothetical field position
and whether a turnover on downs occurs to separate the value of a
play from the air yards versus the yards after catch. For each completed
passing play, we break the estimation of \(EP\) and \(WP\)
into two plays -- one comprising everything leading up to the catch, and
one for the yards after the catch. Because the models rely on the
seconds remaining in the game, we make an adjustment to the time
remaining by subtracting the average length of time for incomplete
passing plays, 5.7
seconds\footnote{This estimate could be improved in future work if information about the time between the snap and the pass becomes available.}.
We then use the \(EP\) or \(WP\) through the air as \(\boldsymbol{V}_f\)
in \autoref{play-value} to estimate \(EPA_{i,air}\) or \(WPA_{i,air}\),
denoting these as \(\delta_{f,i,air}\). We estimate the value of yards
after catch, \(\delta_{f,i,yac}\), by taking the difference between the
value of the following play, \(\boldsymbol{V}_f\), and the value of the
air yards, \(\delta_{f,i,air}\).  We use this to calculate both \(EPA_{i,yac}\) and \(WPA_{i,yac}\).

\section{Evaluating Players with nflWAR}
\label{sec:nflwar}

We use the play values calculated in Section
\ref{sec:ep_wp_model} as the basis for a statistical estimate of wins
above replacement (\textit{WAR}) for each player in the NFL. To do this, we take
the following approach:

\begin{itemize}
\tightlist
\item
  estimate the value of each play (Section \ref{sec:ep_wp_model}),
\item
  estimate the effect of each player on play value added (Section
  \ref{sec:war_model}),
\item
  evaluate relative to replacement level (Section \ref{sec:repl_level}),
\item
  convert to a wins scale (Section \ref{sec:win_conversion}), and
\item
  and estimate the uncertainty in \textit{WAR} (Section \ref{sec:resample}).
\end{itemize}

This framework can be applied to any individual season, and we present
results for the 2017 season in Section \ref{results}. Due to data
restrictions, we currently are only able to produce \textit{WAR} estimates for
offensive skill position players. However, a benefit
of our framework is the ability to separate a player's total value into
the three components of \(WAR_{air}\), \(WAR_{yac}\), and
\(WAR_{rush}\). Additionally, we provide the first statistical estimates for a team's rush blocking based on play-by-play data.

\subsection{Division of Credit}
\label{sec:war_model}

In order to properly evaluate players, we need to allocate the portion
of a play's value \(\delta_{f,i}\) to each player on the field.
Unfortunately, the NFL does not publicly specify which players are on
the field for every play, preventing us from directly applying
approaches similar to those used in basketball and hockey discussed in
Section \ref{sec:prev-work-players}, where the presence of each player on
the playing surface is treated as an indicator covariate in a linear
model that estimates the marginal effect of that player on some game
outcome \citep{Kubatko07, Macdonald11, Thomas13}. Instead, the data
available publicly from the NFL and obtained via \texttt{nflscrapR} are
limited to only those players directly involved in the play, plus
contextual information about the play itself. 

For rushing plays, this includes at the player level the rusher and/or tackler(s), with contextual information for the run gap (end, tackle, guard, middle) and direction (left, middle, right). Further details regarding the nomenclature of run gaps are in our supplementary materials. For passing plays, player level information includes the passer, targeted receiver, tackler(s), and/or interceptor, along with contextual information about the air yards, yards after catch, pass location (left, middle, right), and if the passer was hit on the play.

\hypertarget{multilevel-modeling}{%
\subsubsection{Multilevel Modeling}\label{multilevel-modeling}}

All players in the NFL belong to positional groups that dictate how they
are used in the context of the game. For example, for passing plays we
have the QB and the targeted receiver. However, over the course of an
NFL season, the average QB will have more pass attempts than the average
receiver will have targets, because there are far fewer QBs (more than
60 with pass attempts in the 2017 NFL season) compared to receivers
(more than 400 targeted receivers in the 2017 season).

Because of these systematic differences across positions, there are
differing levels of variation in each position's performance. Additionally, since every play involving the same player is
a repeated measure of performance, the plays themselves are not
independent.  To account for these structural features of football, we use
multilevel models (also referred to as hierarchical, random-effects, or
mixed-effects models), which embrace this positional group structure and
account for the observation dependence. Multilevel models have recently
gained popularity in baseball statistics due to the development of
catcher and pitcher metrics \citep{Brooks15, Turkenkopf15}, but have been used in sports dating back
at least to 2012 \citep{Cafarelli12}. Here, we extend their use for
assessing offensive player contributions in football, using the play
values \(\delta_{f,i}\) from Section \ref{sec:ep_wp_model} as the
response.

In order to arrive at individual player effects we use
varying-intercepts for the groups involved in a play. A simple example
of modeling \(\delta_{f,i}\) with varying-intercepts for two groups, QBs
as \(Q\) and receivers as \(C\), with covariates $X_i$ and coefficients $\beta$ is
\begin{equation}
\label{ex_model_top_level}
\delta_{f,i} \sim N(Q_{q[i]} + C_{c[i]} + X_i \cdot \beta,\ \sigma_{\delta}^2),\ \mbox{for}\ i\ =\ 1,\hdots,n\  \mbox{plays},
\end{equation}

\noindent where the key feature distinguishing multilevel regression from
classical regression is that the group coefficients vary according to
\begin{gather}
          Q_q \sim N(\mu_{Q},\ \sigma_{Q}^2),\ \mbox{for}\ q\ =\ 1,\hdots, \mbox{\#\ of\ QBs},\nonumber \\
          C_c \sim N(\mu_{C},\ \sigma_{C}^2),\ \mbox{for}\ c\ =\ 1,\hdots, \mbox{\#\ of\ receivers}.
\end{gather}

By assigning a probability distribution (such as the normal distribution) to the group intercepts, \(Q_q\) and \(C_c\), with parameters estimated from the data (such as \(\mu_{Q}\) and \(\sigma_{Q}\) for passers), each estimate is pulled toward their respective group mean levels \(\mu_{Q}\) and \(\mu_{C}\). In this example, QBs and receivers involved in fewer plays will be pulled closer to their overall group averages as compared to those involved in more plays and thus carrying more information, resulting in partially pooled estimates \citep{Gelman07}. This approach provides us with average
individual effects on play value added while also providing the
necessary shrinkage towards the group averages. All models we use for
division of credit are of this varying-intercept form, and are fit using penalized likelihood via the \texttt{lme4} package in \texttt{R} \citep{lme4}. While these models are not explicitly Bayesian, as \citet{Gelman07} write, ``[a]ll multilevel models are Bayesian in the sense of assigning probability distributions to the varying regression coefficients", meaning that we are taking into consideration all members of the group when estimating the varying intercepts rather than just an individual effect. 

Our assumption of normality for \(\delta_{f,i}\) follows from our focus on \(EPA\) and \(WPA\) values, which can be both positive and negative, exhibiting roughly symmetric distributions\footnote{Residual plots for models from the 2017 season are available in our supplementary materials.}.  We refer to an intercept estimating a player's average effect as their \emph{individual
points/probability added} (\(iPA\)), with points for modeling \(EPA\)
and probability for modeling \(WPA\). Similarly, an intercept estimating
a team's average effect is their \emph{team points/probability added}
(\(tPA\)). Tables \ref{table-pv-vars} and \ref{table-groups} provide the
notation and descriptions for the variables and group terms in the
models apportioning credit to players and teams on plays. The variables
in Table \ref{table-pv-vars} would be represented by \(X\), and their
effects by \(\beta\) in \autoref{ex_model_top_level}.

\begin{table}
\centering
\caption{Description of variables in the models assessing player and team effects.}
\label{table-pv-vars}
\begin{tabular}{ p{3cm} p{9cm}}
\hline \\ [-1.5ex]
Variable name & Variable description \\ [1ex]
\hline \\ [-1.5ex]
Home & Indicator for if the possession team was home \\ [1ex]
Shotgun & Indicator for if the play was in shotgun formation \\ [1ex]
NoHuddle & Indicator for if the play was in no huddle \\ [1ex]
QBHit & Indicator for if the QB was hit on a pass attempt \\  [1ex]
PassLocation & Set of indicators for if the pass location was either middle or right (reference group is left) \\ [1ex]
AirYards & Orthogonal distance in yards from the line of scrimmage to where the receiver was targeted or caught the ball \\ [1ex]
RecPosition & Set of indicator variables for whether the receiver's position was either TE, FB, or RB (reference group is WR) \\ [1ex]
RushPosition & Set of indicator variables for whether the rusher's position was either FB, WR, or TE (reference group is RB) \\ [1ex]
PassStrength & EPA per pass attempt over the course of the season for the possession team \\ [1ex]
RushStrength & EPA per rush attempt over the course of the season for the possession team \\ [1ex]
\hline
\end{tabular}
\end{table}

\begin{table}
\centering
\caption{Description of groups in the models assessing player and team effects.}
\label{table-groups}
\begin{tabular}{ p{2cm} p{2cm} p{8cm} }
\hline \\ [-1.5ex]
Group & Individual & Description \\ [1ex]
\hline \\ [-1.5ex]
$Q$ & $q$ & QB attempting a pass or rush/scramble/sack \\ [1ex]
$C$ & $c$ & Targeted receiver on a pass attempt \\ [1ex] 
$H$ & $\iota$ & Rusher on a rush attempt \\ [1ex]
$T$ & $\tau$ & Team-side-gap on a rush attempt, combination of the possession team, rush gap and direction \\ [1ex] 
$F$ & $\nu$ & Opposing defense of the pass \\ [1ex]
\hline
\end{tabular}
\end{table}

\subsubsection{Passing Models}

Rather than modeling the \(\delta_{f,i}\) (\(EPA\) or \(WPA\))
for a passing play, we take advantage of the availability of air yards
and develop two separate models for \(\delta_{f,i,air}\) and
\(\delta_{f,i,yac}\). We do not credit the passer solely for the value
gained through the air, nor the receiver solely for the value gained
from after the catch. Instead, we propose that the passer, receiver,
and opposing defense should each have credit divided amongst them
for both areas. We let \(\Delta_{air}\) and
\(\Delta_{yac}\) be the response variables for the air yards and yards
after catch models, respectively. Both models consider all passing
attempts, but the response variable depends on the model 
\begin{gather}
\label{pass-value}
\Delta_{air} = \delta_{f,i,air} \cdot \boldsymbol{1}(\mbox{completion}) + \delta_{f,i} \cdot \boldsymbol{1}(\mbox{incompletion}), \nonumber \\
\Delta_{yac} = \delta_{f,i,yac} \cdot \boldsymbol{1}(\mbox{completion}) + \delta_{f,i} \cdot \boldsymbol{1}(\mbox{incompletion}),
\end{gather}

\noindent where \(\boldsymbol{1}(\mbox{completion})\) and
\(\boldsymbol{1}(\mbox{incompletion})\) are indicator functions for
whether or not the pass was completed. This serves to assign all
completions the \(\delta_{f,i,air}\) and \(\delta_{f,i,yac}\) as the
response for their respective models, while incomplete passes are
assigned the observed \(\delta_{f,i}\) for both models. In using this
approach, we emphasize the importance of completions, crediting accurate
passers for allowing their receiver to gain value after the catch.

The passing model for \(\Delta_{air}\) is 
\begin{gather}
          \Delta_{air} \sim N(Q_{air,q[i]} + C_{air,c[i]} + F_{air,\nu[i]} + \boldsymbol{A}_i \cdot \boldsymbol{\alpha},\ \sigma_{\Delta_{air}})\ \mbox{for}\ i\ =\ 1,\hdots,\ n\ \mbox{plays},\nonumber \\
          Q_{air,q} \sim N(\mu_{Q_{air}},\sigma_{Q_{air}}^2),\ \mbox{for}\ q\ =\ 1,\hdots, \mbox{\#\ of\ QBs},\nonumber \\
          C_{air,c} \sim N(\mu_{C_{air}},\sigma_{C_{air}}^2),\ \mbox{for}\ c\ =\ 1,\hdots, \mbox{\#\ of\ receivers}, \\
          F_{air,\nu} \sim N(\mu_{F_{air}},\sigma_{F_{air}}^2),\ \mbox{for}\ \nu\ =\ 1,\hdots, \mbox{\#\ of\ defenses},\nonumber
\end{gather}

\noindent where the covariate vector \(\boldsymbol{A}_i\) contains a set
of indicator variables for Home, Shotgun, NoHuddle, QBHit, Location,
RecPosition, as well as the RushStrength value while
\(\boldsymbol{\alpha}\) is the corresponding coefficient vector. The
passing model for \(\Delta_{yac}\) is: 
\begin{gather}
\Delta_{yac} \sim N(Q_{yac,q[i]} + C_{yac,c[i]} + F_{yac,\nu[i]} + \boldsymbol{B}_i \cdot \boldsymbol{\beta},\ \sigma_{\Delta_{yac}})\ \mbox{for}\ i\ =\ 1,\hdots,\ n\  \mbox{plays},\nonumber \\
Q_{yac,q} \sim N(\mu_{Q_{yac}},\ \sigma_{Q_{yac}}^2),\ \mbox{for}\ q\ =\ 1,\hdots, \mbox{\#\ of\ QBs},\nonumber \\
          C_{yac,c} \sim N(\mu_{C_{yac}},\ \sigma_{C_{yac}}^2),\ \mbox{for}\ c\ =\ 1,\hdots, \mbox{\#\ of\ receivers}, \\
          F_{yac,\nu} \sim N(\mu_{F_{yac}},\ \sigma_{F_{yac}}^2),\ \mbox{for}\ \nu\ =\ 1,\hdots, \mbox{\#\ of\ defenses},\nonumber
\end{gather}

\noindent where the covariate vector \(\boldsymbol{B}_i\) contains the
same set of indicator variables in \(\boldsymbol{A}_i\) but also
includes the AirYards and interaction terms between AirYards and the
various RecPosition indicators, with \(\boldsymbol{\beta}\) as its
respective coefficient vector. We include the RushStrength in the
passing models as a group-level predictor to control for the possession
team's rushing strength and the possible relationship between the two
types of offense. For QBs, their estimated \(Q_{air,q}\) and
\(Q_{yac,q}\) intercepts represent their \(iPA_{air}\) and \(iPA_{yac}\)
values respectively (same logic applies to receivers). Likewise, the
opposing defense values of \(F_{air,\nu}\) and \(F_{yac,\nu}\) are their
\(tPA_{air}\) and \(tPA_{yac}\) values.

\hypertarget{rushing-models}{%
\subsubsection{Rushing Models}\label{rushing-models}}

For rushing plays, we again model the play values \(\delta_{f,i}\).
However, we build two separate models, with one rushing model for QBs
and another for all non-QB rushes. This is because we cannot consistently separate
(in the publicly available data) designed QB rushes from scrambles on
broken plays, the characteristics of which result in substantially
different distributions of play value added. It is safe to assume all
non-QB rushes are designed rushes. Our rushing model for QBs consists of
all scrambles, designed runs, and sacks (to account for skilled rushing
QBs minimizing the loss on sacks). The QB rushing model is
\begin{gather}
          \delta_{f,i} \sim N(Q_{rush,q[i]} + F_{rush_{Q},\ \nu[i]} + \boldsymbol{\Gamma}_i \cdot \boldsymbol{\gamma},\ \sigma_{\delta_{rush_{Q}}})\ \mbox{for}\ i\ =\ 1,\hdots,\ n\ \mbox{plays},\nonumber \\
          Q_{rush,q} \sim N(\mu_{Q_{rush}},\ \sigma_{Q_{rush}}^2),\ \mbox{for}\ q\ =\ 1,\hdots, \mbox{\#\ of\ QBs}, \\
          F_{rush_{Q},\nu} \sim N(\mu_{F_{rush_{Q}}},\ \sigma_{F_{rush_{Q}}}^2),\ \mbox{for}\ \nu\ =\ 1,\hdots, \mbox{\#\ of\ defenses},\nonumber
\end{gather}

\noindent where the covariate vector \(\boldsymbol{\Gamma}_i\) contains
a set of indicator variables for Home, Shotgun, NoHuddle, as well as the
PassStrength variable where \(\boldsymbol{\gamma}\) is the corresponding
coefficient vector.

For the designed rushing plays of non-QBs, we include an additional
group variable \(T\). As detailed in \autoref{table-groups}, \(T\)
serves as a proxy for the offensive linemen or blockers involved in the
rushing attempt. Each team has seven possible \(T\) levels of the form
team-side-gap. For example, the Pittsburgh Steelers (PIT) have the
following levels: PIT-left-end, PIT-left-tackle, PIT-left-guard,
PIT-middle-center, PIT-right-guard, PIT-right-tackle, PIT-right-end. The
non-QB rushing model is
\begin{gather}
          \delta_{f,i} \sim N(H_{\iota[i]} + T_{\tau[i]} + F_{rush,\nu[i]} + \boldsymbol{P}_i \cdot \boldsymbol{\rho},\ \sigma_{\delta_{rush}})\ \mbox{for}\ i\ =\ 1,\hdots,\ n\ \mbox{plays},\nonumber \\
          H_{\iota} \sim N(\mu_{H},\ \sigma_{H}^2),\ \mbox{for}\ \iota\ =\ 1,\hdots, \mbox{\#\ of\ rushers},\nonumber \\
          T_{\tau} \sim N(\mu_{T},\ \sigma_{T}^2),\ \mbox{for}\ \tau\ =\ 1,\hdots, \mbox{\#\ of\ team-side-gaps}, \\
          F_{rush,\nu} \sim N(\mu_{F_{rush}},\ \sigma_{F_{rush}}^2),\ \mbox{for}\ \nu\ =\ 1,\hdots, \mbox{\#\ of\ defenses},\nonumber
\end{gather}

\noindent where the covariate vector \(\boldsymbol{P}_i\) contains a set
of indicator variables for Home, Shotgun, NoHuddle, RushPosition, and
PassStrength, and where \(\boldsymbol{\rho}\) is the corresponding
coefficient vector. The resulting \(Q_{rush,q}\) and \(H_{rush,\iota}\)
estimates are the \(iPA_{rush}\) values for the QB and non-QB rushers,
respectively. Additionally, the \(T_{\tau}\) estimate is the
\(tPA_{rush,side-gap}\) for one of the seven possible side-gaps for the
possession team, while \(F_{rush,\nu}\) and \(F_{rush_{Q},\nu}\) are the
\(tPA_{rush}\) and \(tPA_{rush_Q}\) values for the opposing defense for
non-QB and QB rushes.

\subsubsection{Individual Points/Probability Added}
\label{sec:ipa}

Let \(\kappa_{p,pass}\) and \(\kappa_{p,rush}\) refer to the number of attempts for player \(p\) on passing and rushing plays, respectively. Using an estimated type of \(iPA\) value for a player \(p\) and multiplying by the player's associated number of attempts provides us with an \emph{individual points/probability above average} (\(iPAA_p\)) value.
The three different types of \(iPAA_p\) values for each position are
\begin{gather}
iPAA_{p,air} = \kappa_{p,pass} \cdot iPA_{p,air}, \nonumber \\
iPAA_{p,yac} = \kappa_{p,pass} \cdot iPA_{p,yac}, \\
iPAA_{p,rush} = \kappa_{p,rush} \cdot iPA_{p,air},\nonumber
\end{gather}

\noindent where the values for \(\kappa_{p,pass}\) and
\(\kappa_{p,rush}\) depend on the player's position. For QBs,
\(\kappa_{p,pass}\) equals their number of pass attempts, while
\(\kappa_{p,rush}\) is the sum of their rush attempts, scrambles, and
sacks. For non-QBs \(\kappa_{p,pass}\) equals their number of targets
and \(\kappa_{p,rush}\) is their number of rush attempts. Summing all
three components provides us with player \(p\)'s total individual
points/probability above average, \(iPAA_p\).

\hypertarget{comparing-to-replacement-level}{%
\subsection{Comparing to Replacement
Level}\label{comparing-to-replacement-level}}

\label{sec:repl_level}

As described in Section \ref{sec:prev-work-players}, it is desirable to
calculate a player's value relative to a ``replacement level'' player's
performance. There are many ways to define replacement level. \citet{Thomas15} define a concept called ``poor man's
replacement'', where players with limited playing time are pooled, and a
single effect is estimated in a linear model, which is considered
replacement level. Others provide more abstract definitions of
replacement level, as the skill level at which a player can be acquired
freely or cheaply on the open market \citep{Tango07}.

We take a similar approach to the \textit{openWAR} method, defining
replacement level by using a roster-based approach \citep{Baumer15}, and
estimating the replacement level effects in a manner similar to that of
\citet{Thomas15}. \citet{Baumer15} argue that ``replacement level''
should represent a readily available player that can replace someone
currently on a team's active roster. Due to differences in the number of
active players across positions in football, we define replacement level
separately for each position. Additionally, because of usage for the
different positions in the NFL, we find separate replacement level
players for receiving as compared to rushing. In doing so, we
appropriately handle cases where certain players have different roles.
For example, a RB that has a substantial number of targets but very few
rushing attempts can be considered a replacement level rushing RB, but
not a replacement level receiving RB.

Accounting for the 32 NFL teams and the typical construction of a roster
\citep{Lillibridge13}, we consider the following players to be ``NFL
level'' for each the non-QB positions:
\begin{itemize}
\tightlist
\item
  rushing RBs = \(32 \cdot 3 = 96\) RBs sorted by rushing attempts,
\item
  rushing WR/TEs = \(32 \cdot 1 = 32\) WR/TEs sorted by rushing attempts,
\item
  receiving RBs = \(32 \cdot 3 = 96\) RBs sorted by targets,
\item
  receiving WRs = \(32 \cdot 4 = 128\) WRs sorted by targets,
\item
  receiving TEs = \(32 \cdot 2 = 64\) TEs sorted by targets.
\end{itemize}

Using this definition, all players with fewer rushing attempts or
targets than the NFL level considered players are deemed
replacement level. This approach is consistent with the one taken by
Football Outsiders \citep{Schatz03}. We combine the rushing replacement
level for WRs and TEs because there are very few WRs and TEs with
rushing attempts.

\begin{figure}[!h]
\centering
\framebox{%
  \begin{minipage}{11pc}
      \vspace{1cm}\par
      pos\_play\_involve\_distr.jpeg\par
      \vspace{1cm}
  \end{minipage}}
\caption{Distribution of the proportion of offensive plays a player is directly involved in by position (2009-2017).}
\label{play-distr-pos}
\end{figure}

Due to the nature of QB usage in the NFL, we proceed in a different manner to find replacement level QBs. \autoref{play-distr-pos} displays the distribution of the percentage of
a team's plays in which a player is directly involved (passer, receiver,
or rusher) by position using data from 2009 to 2017. This does not represent the percentage of team snaps by a player, but
rather for a given position that is directly involved in a play, it shows
the distribution of team play percentages for every player of that
position (e.g. New Orleans Saints' RB Alvin Kamara was involved in
38.39\% of all Saints plays that directly involved a RB). While the
distributions for RB, WR, and TE are unimodal and clearly skewed right,
the distributions for QBs are bimodal for each season. This is an
unsurprising result, since most NFL teams rely on a single QB for an
entire season, resulting in them being involved in more than 80\% of the
team's plays at QB.

Observing this clear difference in the distribution for QBs, we define a replacement level QB as any QB with less than ten percent involvement in their team's plays that directly involve QBs. This approach essentially
asserts that backup QBs with limited playing time should represent
replacement level for QBs, rather than assuming all NFL teams have at
least a certain number of NFL level QBs on their roster. We recognize this definition is far from perfect, we cover an additional ``one QB" approach in our supplementary materials, but we hope this provides a starting point for defining replacement level which researchers can improve upon.

Prior to fitting the models discussed in Section \ref{sec:war_model},
every player who is identified as replacement level is replaced in their
corresponding play-by-play data with their replacement label
(e.g.~Replacement QB, Replacement RB-rushing, Replacement RB-receiving,
etc). By doing so, all replacement level players for a particular
position and type (receiving versus rushing) have the same
\(iPA^{repl}\) estimate. We then calculate a player's value above
replacement, \emph{individual points/probability above replacement}
(\(iPAR_p\)) in the same manner as \citet{Baumer15} and
\citet{Thomas15}, by calculating a replacement level ``shadow'' for a
particular player. For a player \(p\), this is done by first calculating
their replacement ``shadow'' value, \(iPAA_p^{repl}\), by using their respective number of attempts: 
\begin{gather}
  iPAA^{repl}_{p,air} = \kappa_{p,pass} \cdot iPA^{repl}_{air},\nonumber \\
  iPAA^{repl}_{p,yac} = \kappa_{p,pass} \cdot iPA^{repl}_{yac},\\
  iPAA^{repl}_{p,rush} = \kappa_{p,rush} \cdot iPA^{repl}_{rush},\nonumber
\end{gather}

\noindent which leads to natural calculations for the three \(iPAR\)
values: 
\begin{gather}
  iPAR_{p,air} = iPAA_{p,air} - iPAA^{repl}_{p,air},\nonumber \\
  iPAR_{p,yac} = iPAA_{p,yac} - iPAA^{repl}_{p,yac},\\
  iPAR_{p,rush} = iPAA_{p,rush} - iPAA^{repl}_{p,rush}.\nonumber
\end{gather}

\noindent Taking the sum of the three, we arrive at a player's total
\(iPAR_p\).

\subsection{Conversion to Wins}
\label{sec:win_conversion}

If the play's value used for modeling purposes was \(WPA\) based, then
the final \(iPAR\) values are an individual's win probability added above
replacement, which is equivalent to their \emph{wins above replacement}
(\(WAR\)).  However, for the \(EPA\)-based play value response, the \(iPAR\)
values represent the individual expected points added above replacement, and thus
require a conversion from points to wins.  While other, more complicated approaches exist for addressing this (see \cite{Baumer15} for a review), we take a simple
approach, similar to that of \citet{Zhou17} and others:  we use linear regression to estimate the relationship
between team \(t\)'s regular season win total and their score
differential (\(S\)) during the season, \begin{equation}
Wins_t = \beta_0 + \beta_{S}S_t + \epsilon_t,\text{ where } \epsilon_t 
\overset{iid}{\sim} N(0, \sigma^2)\ .
\end{equation}

The resulting coefficient estimate \(\hat{\beta}_{S}\) (typically about 0.03, depending on the season) represents the increase in the number of wins for each one point increase in score differential. Since one additional point of score differential raises the expected number of wins by 0.03, then roughly 33 additional points will raise the expected number of wins by 1.  We can now estimate \(WAR\) for the \(EPA\) based approach by taking the \(iPAR\) values and dividing by 33, the estimated points per win. This is equivalent to multiplying \(iPAR\) by \(\hat{\beta}_{S}\).

%Thus we take the reciprocal, \(\frac{1}{\hat{\beta}_{S}}\) to arrive at the number of points per win. We estimate \(WAR\) for the \(EPA\) based approach by taking the \(iPAR\) values and dividing by the estimated points per win (equivalent to multiplying \(iPAR\) by \(\hat{\beta}_{S}\)). 

\subsection{Uncertainty}
\label{sec:resample}

Similar to the approach taken by \citet{Baumer15} for estimating the
variability in their \emph{openWAR} metric, we use a resampling strategy
to generate distributions for each individual player's \(WAR\) values.
Rather than resampling plays in which a particular player is involved
to arrive at estimates for their performance variability, we resample
entire team drives.  We do this to account for the fact that player usage
is dependent on team decision making, meaning that the random variation
in individual events is dependent upon the random variation in team
events.  Thus, we must resample at the team level to account for the
variability in a player's involvement. The decision to resample whole
drives instead of plays is to represent sampling that is more realistic
of game flows due to the possibility of dependencies within a drive with
regards to team play-calling. In Section \ref{results}, all uncertainty estimation uses this drive-resampling approach, with 1000 simulated seasons.


\section{Results}
\label{results}

Given the definitions in Section \ref{sec:repl_level}, we found the following replacement level designations for the 2017 NFL season:
\begin{itemize}
\tightlist
\item
  rushing:  52 of the 148 RBs are replacement level,
\item
  rushing:  278 of the 310 WR/TEs are replacement level,
\item
  receiving:  52 of the 148 RBs are replacement level,
\item
  receiving:  73 of the 201 WRs are replacement level,
\item
  receiving:  45 of the 109 TEs are replacement level,
\item
  passing:  25 of the 71 QBs are replacement level.
\end{itemize}

We compare the distributions for both types of \(WAR\) estimates,
\(EPA\)-based and \(WPA\)-based, by position in \autoref{war-distr}. For
all positions, the \(EPA\)-based \(WAR\) values tend be higher than the
\(WPA\)-based values. This could be indicative of a player performing
well in meaningless situations due to the score differential,
particularly for QBs.  It is clear that QBs have larger \(WAR\) values
than the other positions, reflecting their involvement in every passing
play and potentially providing value by rushing.  Although this coincides with conventional wisdom regarding the importance of the QB position,
we note that we have not controlled for all possible contributing factors, such as the specific offensive linemen, the team's offensive schemes, or 
the team's coaching ability due to data limitations.  Researchers with
access to this information could easily incorporate their proprietary data into this framework to reach a better assessment of QB value. 

\begin{figure}[!h]
\centering
\framebox{%
  \begin{minipage}{10pc}
      \vspace{1cm}\par
      war\_position\_distr.jpeg\par
      \vspace{1cm}
  \end{minipage}}
%% A small box in place of a figure
\caption{Distribution of \textit{WAR} in 2017 season by type and position.}
\label{war-distr}
\end{figure}

Following Major League Baseball's 2017 MVP race, \(WAR\) has received
heavy criticism for its unclear relationship with wins
\citep{James17, Tango17}.  For this reason, we focus on the \(WPA\)-based
version of \(WAR\), with its direct relationship to winning games.
\autoref{war-bars} displays the top five players based on total \(WAR\)
for each position in the 2017 season.  Each chart is arranged in
descending order by each player's estimated \textit{WAR}, and displays the three separate \(WAR\) values of \(WAR_{air}\), \(WAR_{yac}\), and
\(WAR_{rush}\). By doing this separation, we can see how certain types
of players vary in their performances. Tom Brady for instance is the only
QB in the top five with negative \(WAR_{rush}\).  Alvin Kamara
appears to be providing roughly equal value from rushing and receiving,
while the other top RB performances are primarily driven by rushing success.

\begin{figure}[!h]
\centering
\framebox{%
  \begin{minipage}{11pc}
      \vspace{1cm}\par
      war\_top\_five\_position.jpeg\par
      \vspace{1cm}
  \end{minipage}}
%% A small box in place of a figure
\caption{Top five players in \textit{WAR} by position for the 2017 season.}
\label{war-bars}
\end{figure}

Elaborating on this separation of types of players, we can use the random
intercepts from the multilevel models, the \(iPA\) values, to see the underlying structure of players in terms of their efficiency.  Figures \ref{qb-ipa-plots} and \ref{rb-ipa-plots}
reveal the separation of types of QBs and RBs respectively.  The origin points for both charts represent league averages.  For QBs, we plot their estimates for \(iPA_{air}\) against \(iPA_{yac}\), providing an overview of the types of passers in the NFL. The two components represent different skills of being able to provide value by throwing deep passes through the air, such as Jameis Winston, as compared to short but accurate passers such as Case Keenum.  We can also see where the replacement level QB estimates place for context.  For RBs, we add together their \(iPA_{air}\) and \(iPA_{yac}\) estimates to summarize their individual receiving effect and plot this against their \(iPA_{rush}\) estimates.  This provides a separation between RBs that provide value as receivers versus those who provide positive value primarily from rushing, such as Ezekiel Elliott.  New Orleans Saints RB Alvin Kamara stands out from the rest of the league's RBs, providing elite value in both areas.

\begin{figure}[!h]
\centering
\framebox{%
  \begin{minipage}{9pc}
      \vspace{1cm}\par
      qb\_air\_yac\_plot.jpeg\par
      \vspace{1cm}
  \end{minipage}}
\caption{Estimates for 2017 QB efficiency from \(iPA_{air}\) against \(iPA_{yac}\).}
\label{qb-ipa-plots}
\end{figure}

\begin{figure}[!h]
\centering
\framebox{%
  \begin{minipage}{9pc}
      \vspace{1cm}\par
      rb\_rush\_pass\_plot.jpeg\par
      \vspace{1cm}
  \end{minipage}}
\caption{Estimates for RB efficiency from receiving (\(iPA_{air}\ +\ iPA_{yac}\)) against rushing (\(iPA_{rush}\)) for the 2017 season.}
\label{rb-ipa-plots}
\end{figure}


Using the drive resampling approach outlined in Section \ref{sec:resample},
we can compare the variability in player performance based on
1000 simulated seasons.  \autoref{qb-war-sims} compares the simulation
distributions of the three types of \(WAR\) values (\(WAR_{air}\),
\(WAR_{yac}\), \(WAR_{rush}\)) for selected QBs in the 2017 NFL season,
with a reference line at 0 for replacement level.  We can clearly see
that the variability associated with player performance is not constant,
which is not suprising given the construction of the resampling at the
drive level.  However, we can see some interesting features of QB
performances, such as how Seattle Seahawks QB Russell Wilson's three
types of \(WAR\) distributions are overlapping significantly, emphasizing
his versatility.  Additionally, New England Patriots QB Tom Brady
displays large positive \(WAR_{air}\) and \(WAR_{yac}\) values, but a
clearly negative \(WAR_{rush}\) value.  Finally, Joe Flacco's 2017 performance was at or below replacement level in the vast majority of simulations across all three types of \textit{WAR}, indicating that he is not elite.

\begin{figure}[!h]
\centering
\framebox{%
  \begin{minipage}{8pc}
      \vspace{1cm}\par
      qb\_sim\_distr.jpeg\par
      \vspace{1cm}
  \end{minipage}}
\caption{Simulation distributions of 2017 \textit{WAR} by type for a selection of 12 QBs.}
\label{qb-war-sims}
\end{figure}

\autoref{rb-war-sims} displays the simulation distributions for the top
ten RBs during the 2017 NFL season, as ranked by their average total \(WAR\) across all simulations. Relative to the \(WAR\) values for QBs in \autoref{rb-war-sims}, the best RBs in the league are providing limited value to their teams. This is in agreement with the recent trend of NFL teams, who have been paying QBs increasing salaries but compensating RBs less \citep{Morris17}. Two of
the top RBs in the 2017 were rookies Alvin Kamara and Kareem Hunt,
leading to discussion of which player deserved to be the NFL's
rookie of the year. Similar to \citet{Baumer15} we address this question
using our simulation approach and display the joint distribution of the
two player's 2017 performances in \autoref{hunt-kam-comp}. In nearly
71\% of the simulated seasons, Kamara leads Hunt in \(WAR\) providing us
with reasonable certainty in Kamara providing more value to his team
than Hunt in his rookie season. It should not come as a surprise that
there is correlation between the player performances as each simulation
consists of fitting the various multilevel models resulting in new
estimates for the group averages, individual player intercepts as well
as the replacement level performance.

\begin{figure}[!h]
\centering
\framebox{%
  \begin{minipage}{10pc}
      \vspace{1cm}\par
      top\_rb\_sim\_distr.jpeg\par
      \vspace{1cm}
  \end{minipage}}
\caption{Simulation distributions of 2017 \textit{WAR} value by type for top 10 RBs.}
\label{rb-war-sims}
\end{figure}

\begin{figure}[!h]
\centering
\framebox{%
  \begin{minipage}{10pc}
      \vspace{1cm}\par
      hunt\_kamara\_sim.jpeg\par
      \vspace{1cm}
  \end{minipage}}
%% A small box in place of a figure
\caption{Joint distribution of \textit{WAR} for Alvin Kamara and Kareem Hunt in 2017.}
\label{hunt-kam-comp}
\end{figure}

Additionally, we examine the consistency of the \(WPA\)-based \(WAR\)
from season-to-season based on the correlation within players
between their 2016 and 2017 seasons (excluding replacement level) and
compare this to other commonly used statistics for QBs and RBs. Seen in
\autoref{table-qb-stats}, our estimates for QB \(WAR\) displayed higher
correlations than both the commonly used passer rating statistic as well
as ANY/A.  We also see
higher correlations for RB \(WAR\) as compared to Brian Burke's success
rate (percentage of rush attempts with \(EPA\) greater than zero) and
rushing yards per attempt.  Future work should consider a proper review
and assessment of football statistics accounting for the number of
attempts needed for determing the reliability of a statistic as well as
accounting for when a player changes teams \citep{Yurko17}, and also
apply the framework laid out by \citet{Franks17}.

\begin{table}
\centering
\caption{Correlation of QB statistics between 2016-17 seasons.}
\label{table-qb-stats}
\begin{tabular}{ c c c c}
\hline \\ [-1.5ex]
 & \textit{WAR} & Passer Rating & ANY/A \\ [1ex]
\hline \\ [-1.5ex]
Correlation & 0.598 & 0.478 & 0.295 \\ [1ex]
\hline
\end{tabular}
\end{table}

\begin{table}
\centering
\caption{Correlation of RB statistics between 2016-17 seasons.}
\label{table-rb-stats}
\begin{tabular}{ c c c c}
\hline \\ [-1.5ex]
 & \textit{WAR} & Success Rate & Yards per Attempt \\ [1ex]
\hline \\ [-1.5ex]
Correlation & 0.431 & 0.314 & 0.337 \\ [1ex]
\hline
\end{tabular}
\end{table}

Although it does not provide a measure for individual players'
contributions, we can sum together the seven possible
\(tPA_{rush,side-gap}\) estimates for a team providing a proxy for their
offensive line's overall efficiency in contributing to rushing plays.
We can also look at individual side-gaps for specific teams to assess
their offensive line's performance in particular areas.  
\autoref{oline-plot} displays the \(tPA_{rush,side-gap}\) sum in 2017
against 2016 for each NFL team.  The red lines provide indication to
average performances in each year, so teams in the upper right quadrant
performed above average overall in both years such as the Dallas Cowboys
(DAL) which are known to have one of the best offensive lines in
football.  

\begin{figure}[!h]
\centering
\framebox{%
  \begin{minipage}{10pc}
      \vspace{1cm}\par
      oline\_tpa\_plot.jpeg\par
      \vspace{1cm}
  \end{minipage}}
%% A small box in place of a figure
\caption{Team offensive line measures.}
\label{oline-plot}
\end{figure}

\section{Discussion and Extensions}
\label{sec:discussion}

In this work, we have provided four major contributions to the statistical analysis of NFL football, in areas that can impact both on-field and player personnel decisions.  We discuss these contributions and some extensions below.

\subsection{Reproducible Play and Player Evaluation}

\textbf{Data and Software Development}:  We provide an \texttt{R} package, \texttt{nflscrapR}, to provide easy access to publicly available NFL play-by-play data for researchers to use in their own analyses of the NFL.  This package has already been used by researchers to further research into NFL decision-making \citep{Yam18}.

\vspace{4mm}

\noindent \textbf{Play Evaluation}:  We make two contributions in the area of play evaluation.  First, we introduce a novel approach for estimating expected points using a multinomial logistic regression model that is fully reproducible.  Second, we use a generalized additive model for estimating in-game win probability, incorporating the results of the expected points model as input.  With these two play evaluation models, we can calculate measures such as expected points added and win probability added, which are commonly used to evaluate both plays and players.  All of these measures are included directly into the play-by-play data provided by \texttt{nflscrapR}.  Moreover, all code used to build these expected points and win probability models is provided in \texttt{nflscrapR} and available on GitHub \url{https://github.com/ryurko/nflscrapR-models}.  By taking these important steps, we ensure that all of our methods are fully reproducible, and we make it as easy as possible for researchers to use, explore, and improve upon our work. 

\vspace{4mm}

\noindent \textbf{Player Evaluation}:  With our \textit{nflWAR} framework, we use multilevel models to isolate offensive skill player contribution and estimate their individual wins above replacement.  

Our estimates of \textit{WAR} are given for several different areas of the game and are available for all offensive skill position players, unlike previous approaches.  By compartmentalizing our estimates of player \textit{WAR}, we are able to better characterize players and how they achieved success.  For example, New Orleans Saints RB Alvin Kamara was unique in his success as both a rusher and a receiver in the 2017 NFL season.  Similarly, Seattle Seahawks QB Russell Wilson was unique in his success as a rusher as well as from passing through the air and for yards after the catch, with about equal \textit{WAR} contributions in all three areas in the 2017 NFL season.  While these findings may not surprise knowledgeable football fans, our framework also reveals the value of potentially overlooked skills, such as the rushing ability of Tyrod Taylor and Dak Prescott, as seen in \autoref{qb-war-sims}.The value they provide by their rushing WAR reflects not only their ability to scramble, but their ability to limit the loss from sacks as compared to other QBs. This is a skill that cannot be captured with basic statistics such as sack rate (which treats all sacks as equal).

Our multilevel modeling approach provides the first statistical estimate of an offensive line's value towards run-blocking that also controls for factors such as RB ability, opposing defense, etc.  We recognize, however, that this is not a perfect measure of offensive line performance since it does not necessarily capture individual linemen, and does not account for potential selection bias that could influence specific side-gap estimates (since RBs are likely to run towards holes and away from defenders).  We lack information about which specific offensive linemen are on the field or even involved in plays, preventing us from fitting player-specific terms in our multilevel model that would provide \textit{WAR} estimates for individual offensive linemen.  Researchers with access to this data can build this into our modeling framework with minimal issues, as we discuss in Section \ref{sec:road_to_war}.  %However, until more data becomes available, researchers can incorporate these measures with more nuanced approaches of measuring offensive line performance such as \citet{Alamar08} and \citet{Alamar11}.

Adopting a resampling procedure similar to that of \citet{Baumer15}, we provide estimates of uncertainty on all \textit{WAR} estimates.  Our approach resamples at the drive-level, rather than individual plays, to preserve the effects of any within-drive factors, such as play sequencing or situational play-calling tendencies.

Finally, our \textit{WAR} models are fully reproducible, with all data coming directly from \texttt{nflscrapR}, and with all code provided on GitHub \url{https://github.com/ryurko/nflWAR}.  %Because we use parametric models, it is trivially easy to incorporate more information, such as information about which players are on the field, or information from player-tracking data.  We encourage future researchers to expand and improve upon our models in future work.

\subsection{Extensions Relevant to NFL Teams}
\label{sec:road_to_war}


\textbf{The Road to WAR for Players at All Positions}:  One key benefit to our approach is that it can easily be augmented with the inclusion of additional data sources, e.g. player-tracking data or proprietary data collected by NFL teams. Given data about which players are present on the field for each play, we can update our multilevel models from Section \ref{sec:war_model} by including additional positional groups.  For example, for the non-QB rushing model, we can update the model as follows:
\begin{gather}
          \delta_{f,i} \sim N(\sum_k O^{k}_{rush,\nu_k[i]} + \sum_g D^{g}_{rush,\nu_g[i]} + \boldsymbol{P}_i \cdot \boldsymbol{\rho},\ \sigma_{\delta_{rush}})\ \mbox{for}\ i\ =\ 1,\hdots,\ n\ \mbox{plays},\nonumber \\
          O^{k}_{rush,\nu_k} \sim N(\mu_{O^{k}_{rush}},\ \sigma_{O^{k}_{rush}}^2), \nonumber \\
          D^{g}_{rush,\nu_g} \sim N(\mu_{D^{g}_{rush}},\ \sigma_{D^{g}_{rush}}^2), \nonumber
\end{gather}

\noindent where \(O^{k}_{rush,\nu_k}\) are the intercepts for offensive positions, indexed by $k$, \(D^{g}_{rush,\nu_g}\) are the intercepts for defensive positions, indexed by $g$, with both types of positions varying according to their own model, where \(\boldsymbol{P}_i\) and \(\boldsymbol{\rho}\) are described as above.  Similar updates can be made to the models representing QB rushing, passing through the air, and passing for yards after catch.  After doing so we can calculate the \(iPAA\) for any player at any position and, with adequate definitions for replacement level at each position, will have statistical \textit{WAR} estimates for players of any position, offensive and defensive.

\vspace{4mm}

\noindent \textbf{Roster Construction}:  If NFL teams have player participation data (detailing which players are on the field for each play) and are able to implement the framework above, they would then have \textit{WAR} estimates for players at all positions dating back as far back as they have complete player participation data.  Teams that are able to do this could potentially gain substantial advantages in important areas of roster construction.

First, teams could more appropriately assess the contract values of players in free agency, similar to what is commonly done in baseball \citep{Paine15b}.  Second and perhaps most importantly, teams would be able to substantially improve their analysis for the NFL draft.  Using an approach similar to that of \citet{Citrone17}, teams could substitute an objective measure of \textit{WAR} in place of the more subjective measure of AV, in order to project the future career value in terms of \textit{WAR} for all players available in the NFL draft.  Additionally, teams employing this approach could create updated, \textit{WAR}-based versions of the ``draft pick value chart'', first attributed to Jimmy Johnson and later improved by \citet{Meers11} and \citet{Citrone17}.  In doing so, teams could more accurately assess the value of draft picks and potentially exploit their counterparts in trades involving draft picks.

%% BibTeX support
\bibliographystyle{DeGruyter}
\bibliography{bibliography}

%%%%%%%%%% Merge with supplemental materials %%%%%%%%%%
\pagebreak
\widetext
\setcounter{page}{1}
\begin{center}
\textbf{\large Supplementary Materials for:\\ \vspace{2cm} ``nflWAR: A Reproducible Method for Offensive Player Evaluation in Football"}
\end{center}
\pagebreak

%%%%%%%%%% Merge with supplemental materials %%%%%%%%%%
%%%%%%%%%% Prefix a "S" to all equations, figures, tables and reset the counter %%%%%%%%%%
\setcounter{equation}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{section}{0}
\makeatletter
\renewcommand{\theequation}{S\arabic{equation}}
\renewcommand{\thefigure}{S\arabic{figure}}
\renewcommand{\bibnumfmt}[1]{[S#1]}
\renewcommand{\citenumfont}[1]{S#1}
%%%%%%%%%% Prefix a "S" to all equations, figures, tables and reset the counter %%%%%%%%%%


\section{Play-by-Play Data with \texttt{nflscrapR}}
\label{sec_sup:data}

Data in professional sports comes in many different forms. At the
season-level, player and team statistics are typically available dating
back to the 1800s \citep[\citet{Phillips}]{Lahman}. At the game-level,
player and team statistics have been tracked to varying degrees of
detail dating back several decades \citep{Lahman}. Within games, data is
available to varying degrees of granularity across sports and leagues.
For example, Major League Baseball (MLB) has play-by-play data at the
plate appearance level available dating back several decades
\citep{Lahman}, while the National Hockey League (NHL) only began
releasing play-by-play via their real-time scoring system in the 2005-06
season \citep{Thomas17}.

Play-by-play data, or information specifying the conditions, features,
and results of an individual play, serves as the basis for most modern
sports analysis in the public sphere \citep[\citet{Macdonald11},
\citet{Lock14}, \citet{Thomas17}]{Kubatko07}. Outside of the public
sphere, many professional sports teams and leagues have access to data
at even finer levels of granularity, e.g.~via optical player tracking
systems in the National Basketball Association, MLB, and the English
Premier League that track the spatial distribution of players and
objects at multiple times per second. The NFL in 2016 began using
radio-frequency identification (RFID) technology to track the locations
of players and the football \citep{CBS}, but as of mid 2018, this data
is not available publicly, and NFL teams have only just gained accessed to the data beyond their own players. In almost all major professional sports leagues, play-by-play data is provided and includes information on in-game
events, players involved, and (usually) which players are actively
participating in the game for each event
\citep[\citet{Lahman}]{Thomas17}.

Importantly, this is not the case for the NFL. While play-by-play data
is available through the NFL.com application programming interface
(API), the league does not provide information about which players are
present on the playing field for each play, what formations are being
used (aside from the ``shotgun'' formation), player locations, or
pre-snap player movement. This is extremely important, as it limits the
set of players for which we can provide estimates of their contribution
to game outcomes (e.g.~points scored, points allowed, wins, losses,
etc).

We develop an \texttt{R} package \citep{R17}, called \texttt{nflscrapR},
that provides users with clean datasets, box score statistics, and more
advanced metrics describing every NFL play since 2009
\citep{Horowitz17}. This package was inspired largely by other
\texttt{R} packages facilitating the access of sports data. For hockey,
\texttt{nhlscrapR} provides clean datasets and advanced metrics to use
for analysis for NHL fans \citep{Thomas17}. In baseball, the R packages
\texttt{pitchRx} \citep{Sievert15}, \texttt{Lahman} \citep{Lahman}, and
\texttt{openWAR} \citep{Baumer15} provide tools for collecting MLB data
on the pitch-by-pitch level and building out advanced player evaluation
metrics. In basketball, \texttt{ballR} \citep{Elmore17} provides
functions for collecting data from \texttt{basketball-reference.com}.

Each NFL game since 2009 has a 10 digit game identification number (ID)
and an associated set of webpages that includes information on the scoring
events, play-by-play, game results, and other game data. The API
structures its data using JavaScript Object Notation (JSON) into three
major groups: game outcomes, player statistics at the game level, and
play-by-play information. The design of the \texttt{nflscrapR} package
closely mimics the structure of the JSON data in the API, with four main
functions described below:

\texttt{season\_games()}: Using the data structure outputting end of
game scores and team matchups, this function provides end of game
results with an associated game ID and the home and away teams
abbreviations.

\texttt{player\_game()}: Accessing the player statistics object in the
API's JSON data, this function parses the player level game summary data
and creates a box-score-like data frame. Additional functions provide
aggregation functionality:\\ \texttt{season\_player\_game()} binds the
results of \texttt{player\_game()} for all games in a season, and
\texttt{agg\_player\_season()} outputs a single row for each player with
their season total statistics.

\texttt{game\_play\_by\_play()}: This is the most important function in
\texttt{nflscrapR}. The function parses the listed play-by-play data
then uses advanced regular expressions and other data manipulation tasks
to extract detailed information about each play (e.g.~players involved
in action, play type, penalty information, air yards gained, yards
gained after the catch, etc.). The \texttt{season\_play\_by\_play()}
binds the results of \texttt{game\_play\_by\_play()} for all games in a
season.

\texttt{season\_rosters()}: This function outputs all of the rostered
players on a specified team in a specified season and includes their
name, position, unique player ID, and other information.

For visualization purposes we also made a dataset, \texttt{nflteams}
available in the package which includes the full name of all 32 NFL
teams, their team abbreviations, and their primary
colors\footnote{Some of this information is provided through Ben Baumer's \texttt{R} package \texttt{teamcolors} \citep{Baumer17b}}.

In addition to the functions provided in \texttt{nflscrapR}, we provide
downloadable versions in comma-separated-value format, along with a
complete and frequently updating data dictionary, at
\url{https://github.com/ryurko/nflscrapR-data}. The datasets provided on this website included play-by-play from 2009 -- 2017, game-by-game player level statistics, player-season total statistics, and team-season total statistics. These datasets are made available to allow users familiar with other software to do research in the realm of football analytics. Table \ref{table-pbp} gives a brief overview of some of the more important variables used for evaluating plays in Section
\ref{sec:ep_wp_model}.

\begin{table}
\centering
\caption{Description of the play-by-play dataset.}
\label{table-pbp}
\begin{tabular}{p{3cm} p{9cm}}
\hline \\ [-1.5ex]
Variable & Description \\ [1ex]
\hline \\ [-1.5ex]
Possession Team & Team with the ball on offense (opposing team is on defense) \\ [1ex]
Down & Four downs to advance the ball ten (or more) yards \\ [1ex]
Yards to go & Distance in yards to advance and convert first down \\ [1ex]
Yard line & Distance in yards away from opponent's endzone (100 to zero)  \\ [1ex]
Time Remaining & Seconds remaining in game, each game is 3600 seconds long (four quarters, halftime, and a potential overtime) \\ [1ex]
Score differential & Difference in score between the possession team and opposition \\
\hline 
\end{tabular}
\end{table}

\section{Expected Points Model Details}

\label{ep-supplement}

\subsection{Model Variables}

The covariates describing the game situation for each play that are used in our \(EP\) model are displayed in Table \ref{table-ep-vars}.

\begin{table}
\centering
\caption{Description of variables for the $EP$ model.}
\label{table-ep-vars}
\begin{tabular}{ p{3cm} p{9cm}}
\hline \\ [-1.5ex]
Variable & Variable description \\ [1ex]
\hline \\ [-1.5ex]
Down & The current down (1st, 2nd, 3rd, or 4th\\ [1ex]
Seconds & Number of seconds remaining in half \\ [1ex]
Yardline & Yards from endzone (0 to 100)  \\ [1ex]
log(YTG) & Log transformation of yards to go for a first down \\ [1ex]
GTG & Indicator for whether or not it is a goal down situation \\ [1ex]
UTM & Indicator for whether or not time remaining in the half is under two minutes \\ [1ex]
\hline
\end{tabular}
\end{table}

\hypertarget{observation-weighting}{%
\subsection{Observation Weighting}\label{observation-weighting}}

Potential problems arise when building an expected points model
because of the nature of football games. The first issue, as pointed out
by \citet{BurkeEP}, regards the score differential in a game. When a
team is leading by a large number of points at the end of a game they
will sacrifice scoring points for letting time run off the clock. This
means that plays with large score differentials can exhibit a different
kind of relationship with the next points scored than plays with tight
score differentials. Although others such as Burke only use the subset
of plays in the first and third quarter where the score differential is
within ten points, we don't exclude any observations but instead use a
weighting approach. \autoref{score_diff_hist}A displays the distribution
for the absolute score differential, which is clearly skewed right, with a higher proportion of plays possessing smaller score
differentials. Each play \(i \in \{1, \hdots, n\}\), in the modeling data of regular season games from 2009 to 2016, is assigned a weight
\(w_i\) based on the score differential \(S\) scaled from zero to one
with the following function:

\begin{equation}
\label{weight}
w_i = w(S_i) = \frac{\underset{i}{max}(|S_i|) - |S_i|}{\underset{i}{max}(|S_i|) - \underset{i}{min}(|S_i|)}
\end{equation}

In addition to score differential, we also weight plays according to
their ``distance'' to the next score in terms of the number of drives.
For each play \(i\), we find the difference in the number of drives from
the next score \(D\): \(D_i = d_{next\  score} - d_i\), where
\(d_{next\  score}\) and \(d_i\) are the drive numbers for the next
score and play \(i\), respectively. For plays in the first half, we
stipulate that \(D_i = 0\) if the \(d_{next\  score}\) occurs in the
second half, and similarly for second half plays for which the next
score is in overtime. \autoref{score_diff_hist}B displays the
distribution of \(D_i\) excluding plays with the next score as ``No
Score.'' This difference is then scaled from zero to one in the same way
as the score differential in \autoref{weight}. The score differential
and drive score difference weights are then added together and again
rescaled from zero to one in the same manner resulting in a combined
weighting scheme. By combining the two weights, we are placing equal
emphasis on both the score differential and the number of drives until
the next score and leave adjusting this balance for future work.

\begin{figure}[!h]
\centering
\framebox{%
  \begin{minipage}{10pc}
      \vspace{1cm}\par
      distr\_score\_drive.jpeg\par
      \vspace{1cm}
  \end{minipage}}
\caption{Distributions for (A) absolute score differential and (B) number of drives until next score (excluding plays without a next score event).}
\label{score_diff_hist}
\end{figure}

\hypertarget{pats-and-field-goals}{%
\subsection{PATs and Field Goals}\label{pats-and-field-goals}}

\label{sec:pat_fg}

As noted earlier, we treat PATs (extra point attempts and two-point
attempts) separately. For two-point attempts, we simply use the
historical success rate of 47.35\% from 2009-2016, resulting in
\(EP = 2 \cdot 0.4735 = 0.9470\). Extra point attempts use the
probability of successfully making the kick from a generalized additive
model (see Section \ref{gam}) that predicts the probability of making the
kick, \(P(M)\) for both extra point attempts and field goals as a smooth
function of the kick's distance, \(k\) (total of 16,906 extra point and
field goal attempts from 2009-2016):
\begin{equation}
\text{log}(\frac{P(M)}{1-P(M)}) = s(k).
\end{equation}

The expected points for extra point attempts is this predicted
probability of making the kick, since the actual point value of a PAT is
one. For field goal attempts, we incorporate this predicted probability
of making the field goal taking into consideration the cost
of missing the field goal and turning the ball over to the opposing
team. This results in the following override for field goal attempts:
\begin{equation}
EP_{field\ goal\ attempt} = P(M)\cdot 3 + (1 - P(M))\cdot (-1)\cdot E[Y|X=m],
\end{equation}

\noindent where \(E[Y|X=m]\) is the expected points from the multinomial
logistic regression model but assuming the opposing team has taken
possession from a missed field goal, with the necessary adjustments to
field position and time remaining (eight yards and 5.07 seconds,
respectively, estimated from NFL regular season games from 2009 to 2016), and multiplying by
negative one to reflect the expected points for the team attempting the
field goal. Although these calculations are necessary for proper
calculation of the play values $\delta_{f,i}$ discussed in Section
\ref{epa-wpa}, we note that this is a rudimentary field goal model only
taking distance into account. Enhancements could be made with additional
data (e.g.~weather data, which is not made available by the NFL) or by
using a model similar to that of \citet{Morris15}, but these are beyond
the scope of this paper.


\section{Win Probability Example}

An example of a single game \(WP\) chart is provided in
\autoref{wp_example} for the 2017 American Football Conference (AFC)
Wild Card game between the Tennessee Titans and Kansas City Chiefs.  The game starts with both teams having an equal chance of winning, with minor variations until the score differential changes (in this case, in favor of Kansas City). Kansas City led 21-3 after the first half, reaching a peak win probability of roughly 95\% early in the third quarter, before giving up 19 unanswered points in the second half and losing to Tennessee 22-21.

\begin{figure}[!h]
\centering
\framebox{%
  \begin{minipage}{10pc}
      \vspace{1cm}\par
      game\_wp\_chart\_ex.jpeg\par
      \vspace{1cm}
  \end{minipage}}
\caption{Win probability chart for 2017 AFC Wild Card game.}
\label{wp_example}
\end{figure}

\section{Run Gap Explanation}

\autoref{fig:gaps} provides a diagram of the run gaps (in blue) and the
positions along the offensive line (in black). In the NFL play-by-play, the gaps are not referred to with letters, as they commonly are by football players and coaches; instead, the terms ``middle'', ``guard'', ``tackle'', and ``end'' are used. For the purposes of this paper, we define the following linkage between these two nomenclatures:
\begin{itemize}
\tightlist
\item
  ``A'' Gap = ``middle''
\item
  ``B'' Gap = ``guard''
\item
  ``C'' Gap = ``tackle''
\item
  ``D'' Gap = ``end''
\end{itemize}

\begin{figure}[!h]
\centering
\framebox{%
  \begin{minipage}{8pc}
      \vspace{1cm}\par
      run\_gaps\_plot.jpeg\par
      \vspace{1cm}
  \end{minipage}}
%% A small box in place of a figure
\caption{Offensive Line Gaps for Rushing Plays.}
\label{fig:gaps}
\end{figure}

\section{Relationship between Score Differential and Wins}

\autoref{wins-score} displays the estimated linear regression fits from modeling the relationships between the number of regular season wins and score differential for each season from 2009 to 2017.

\begin{figure}[!h]
\centering
\framebox{%
  \begin{minipage}{10pc}
      \vspace{1cm}\par
      win\_score\_rel\_chart.jpeg\par
      \vspace{1cm}
  \end{minipage}}
\caption{Relationship between number of wins and score differential in the regular season by year (2009-2017).}
\label{wins-score}
\end{figure}

\section{WAR Residual Diagnostics}

\autoref{war-resid} displays the residuals against fitted values for each of the four different WAR models fit on data from the 2017 season. There does not appear to be any severe violations of model assumptions. The 2017 season residual plots are consistent with results seen for each of the available seasons dating back to 2009.

\begin{figure}[!h]
\centering
\framebox{%
  \begin{minipage}{11pc}
      \vspace{1cm}\par
      war\_model\_resid\_plots.jpeg\par
      \vspace{1cm}
  \end{minipage}}
\caption{Residuals against fitted values for the four different WAR models using data from the 2017 season.}
\label{war-resid}
\end{figure}

\section{QB Replacement Level}

The second definition we consider for replacement level QB is to limit NFL level to be the 32 QBs that attempted a pass in the first quarter of the first game of the season for each team, and label all remaining QBs as replacement level. The logic here is that NFL teams typically do not sign free agent QBs outside of their initial roster during the course of the season because it takes time to learn a team's playbook and offensive schemes. 

For the 2017 season, the ``ten percent of QB plays cutoff'' approach results 25 replacement level QBs, while the ``one QB for each team'' approach results in 39 replacement level QBs out of the 71 in total. We compare the distributions of both types of \(WAR\) estimates, \(EPA\)-based and \(WPA\)-based, for the two considered definitions of replacement level QBs in \autoref{qb-war-distr}. It is clear that the ``one QB for each team'' approach for defining replacement level leads to lower \(WAR\) values in general, likely because some QBs who begin the season as back-ups perform better than those who begin the season as starters, yet are designated replacement level with this approach.

\begin{figure}[!h]
\centering
\framebox{%
  \begin{minipage}{9pc}
      \vspace{1cm}\par
      war\_qb\_repl\_distr.jpeg\par
      \vspace{1cm}
  \end{minipage}}
%% Use the graphics package to insert figures
%% A small box in place of a figure
\caption{Distribution of QB \textit{WAR} in 2017 season by type and replacement level definition.}
\label{qb-war-distr}
\end{figure}

